Evaluation of Dataframe Libraries for Data Preparation on a Single Machine

Data preparation is a trial-and-error process that typically involves countless iterations over the data to define the best pipeline of operators for a given task. With tabular data, practitioners often perform that burdensome activity on local machines by writing ad hoc scripts with libraries based on the Pandas dataframe API and testing them on samples of the entire dataset-the faster the library, the less idle time its users have. In this paper, we evaluate the most popular Python dataframe libraries in general data preparation use cases to assess how they perform on a single machine. To do so, we employ 4 real-world datasets with heterogeneous features, covering a variety of scenarios, and the TPC-H benchmark. The insights gained with this experimentation are useful to data scientists who need to choose which of the dataframe libraries best suits their data preparation task at hand. In a nutshell, we found that: for small datasets, Pandas consistently proves to be the best choice with the richest API; when data fits in RAM and there is no need for complete compatibility with Pandas API, Polars is the go-to choice thanks to its in-memory execution and query optimizations; when a GPU is available, CuDF often yields the best performance, while for very large datasets that cannot fit in the GPU memory and RAM, PySpark (thanks to a multithread execution and a query optimizer) proves to be the best option.

==> input/images/fig1/fig1_backup.tex <==
\begin{figure*}[ht]

\begin{subfigure}{\textwidth}
         \centering
         \hspace*{0.8cm}\includegraphics[width=0.945\linewidth]{input/images/fig1/legend.pdf}
\end{subfigure}

\begin{subfigure}{\textwidth}
    \begin{subfigure}[b]{0.245\textwidth}
         \centering
         \includegraphics[width=\textwidth]{input/images/fig1/Athlete_EDA.pdf}
         \vspace*{-0.8cm}
         \caption{Athlete, EDA}
         \label{fig:athlete_eda}
    \end{subfigure}
    \hfill
        \begin{subfigure}[b]{0.245\textwidth}
         \centering
         \includegraphics[width=\textwidth]{input/images/fig1/Loan_EDA.pdf}
         \vspace*{-0.8cm}
         \caption{Loan, EDA}
         \label{fig:loan_eda}
    \end{subfigure}
    \hfill
        \begin{subfigure}[b]{0.245\textwidth}
         \centering
         \includegraphics[width=\textwidth]{input/images/fig1/Patrol_EDA.pdf}
                 \vspace*{-0.81cm}
        \caption{Patrol, EDA}
         \label{fig:patrol_eda}
    \end{subfigure}
    \hfill
        \begin{subfigure}[b]{0.245\textwidth}
         \centering
         \includegraphics[width=\textwidth]{input/images/fig1/Taxi_EDA.pdf}
        \vspace*{-0.8cm}
         \caption{Taxi, EDA}
         \label{fig:taxi_eda}
    \end{subfigure}
\end{subfigure}
\hfill
\begin{subfigure}{\textwidth}
    \begin{subfigure}[b]{0.245\textwidth}
         \centering
         \includegraphics[width=\textwidth]{input/images/fig1/Athlete_DT.pdf}
         \vspace*{-0.8cm}
         \caption{Athlete, DT}
         \label{fig:athlete_dt}
    \end{subfigure}
    \hfill
        \begin{subfigure}[b]{0.245\textwidth}
         \centering
         \includegraphics[width=\textwidth]{input/images/fig1/Loan_DT.pdf}
         \vspace*{-0.8cm}
         \caption{Loan, DT}
         \label{fig:loan_dt}
    \end{subfigure}
    \hfill
        \begin{subfigure}[b]{0.245\textwidth}
         \centering
         \includegraphics[width=\textwidth]{input/images/fig1/Patrol_DT.pdf}
         \vspace*{-0.81cm}
         \caption{Patrol, DT}
         \label{fig:patrol_dt}
    \end{subfigure}
    \hfill
        \begin{subfigure}[b]{0.245\textwidth}
         \centering
         \includegraphics[width=\textwidth]{input/images/fig1/Taxi_DT.pdf}
          \vspace*{-0.8cm}
         \caption{Taxi, DT}
         \label{fig:taxi_dt}
    \end{subfigure}
\end{subfigure}
\hfill
\begin{subfigure}{\textwidth}
    \begin{subfigure}[b]{0.245\textwidth}
         \centering
         \includegraphics[width=\textwidth]{input/images/fig1/Athlete_DC.pdf}
        \vspace*{-0.8cm}
         \caption{Athlete, DC}
         \label{fig:athlete_dc}
    \end{subfigure}
    \hfill
        \begin{subfigure}[b]{0.245\textwidth}
         \centering
         \includegraphics[width=\textwidth]{input/images/fig1/Loan_DC.pdf}
        \vspace*{-0.8cm}
         \caption{Loan, DC}
         \label{fig:loan_dc}
    \end{subfigure}
    \hfill
        \begin{subfigure}[b]{0.245\textwidth}
         \centering
         \includegraphics[width=\textwidth]{input/images/fig1/Patrol_DC.pdf}
            \vspace*{-0.81cm}
         \caption{Patrol, DC}
         \label{fig:patrol_dc}
    \end{subfigure}
    \hfill
        \begin{subfigure}[b]{0.245\textwidth}
         \centering
         \includegraphics[width=\textwidth]{input/images/fig1/Taxi_DC.pdf}
        \vspace*{-0.8cm}
        \caption{Taxi, DC}
         \label{fig:taxi_dc}
    \end{subfigure}
\end{subfigure}
\caption{Average runtime for each stage of the data preparation pipeline (EDA, DT, DC) on different datasets.}
\label{fig:avg_stage}
\end{figure*}

==> input/images/fig4/fig4.tex <==
\begin{figure*}[ht]

% \begin{subfigure}{\textwidth}
%          \centering
%          \hspace*{0.4cm}\includegraphics[width=0.97\linewidth]{input/images/fig4/legend.pdf}
% \end{subfigure}

\begin{subfigure}{\textwidth}
    \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{input/images/fig4/scalable0.pdf}
         \vspace*{-0.6cm}
         \caption{Laptop}
         \label{fig:8_16}
    \end{subfigure}
    \hfill
        \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{input/images/fig4/scalable1.pdf}
         \vspace*{-0.6cm}
         \caption{Workstation}
         \label{fig:16_64}
    \end{subfigure}
    \hfill
        \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{input/images/fig4/scalable2.pdf}
                 \vspace*{-0.61cm}
        \caption{Server}
         \label{fig:24_128}
    \end{subfigure}
\end{subfigure}
\caption{
Average runtime for running the entire pipeline on incremental samples of \taxi.\\
{\color{red} 
Rev1D5 Fig 6 shows the time on growing amounts of data, and calls this "scalability", however, the use of a log-linear scale left me unclear which platform grows slowest [though it is clear which is absolutely fastest]. To display scalability, I suggest to chart something like time-on-givendatasize/time-on-standard-size.\\
Rev4(D12) I find that Figures 6 (a) and (b) add relatively little to what is shown in Table 5 and Figure 6 (c). If the authors are looking to save space/cut content, that'd be my first suggestion.\\
Rev4(D13) Maybe a log scale on the y axis of Figure 6 would make the results easier to interpret. (A linear relationship would result in a straight line on this log-log plot, and deviations from that would be easier to spot that on the lin-log plot.)
}
}
\label{fig:scalability}
\end{figure*}

==> input/images/fig4_2/fig4.tex <==
\newcommand{\sv}{\selectfont{\cellcolor[HTML]{f9844a}{\textsf{}\xspace}}}
\newcommand{\pc}{\selectfont{\cellcolor[HTML]{90BE6D}{\textsf{}\xspace}}}
\newcommand{\ws}{\selectfont{\cellcolor[HTML]{FEDC97}{\textsf{}\xspace}}}

\begin{table*}
\begin{minipage}{\columnwidth}
\begin{subfigure}{\textwidth}
         \centering
         \hspace*{0.4cm}\includegraphics[width=0.97\linewidth]{input/images/fig4_2/legend.pdf}
\end{subfigure}
\begin{subfigure}{\textwidth}
    \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=1.11\textwidth]{input/images/fig4_2/scalable0.pdf}
         \vspace*{-0.5cm}
         \caption{Laptop}
         \label{fig:8_16}
    \end{subfigure}
    \hspace{-0.4cm}
    \hfill
        \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{input/images/fig4_2/scalable1.pdf}
         \vspace*{-0.5cm}
         \caption{Workstation}
         \label{fig:16_64}
    \end{subfigure}
    \hspace{-0.7cm}
    \hfill
        \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=1.04\textwidth]{input/images/fig4_2/scalable2.pdf}
                 \vspace*{-0.5cm}
        \caption{Server}
         \label{fig:24_128}
    \end{subfigure}

\end{subfigure}
\label{fig:scalability}
\vspace*{-0.7cm}
\captionof{figure}{
Average runtime for running the entire pipeline on incremental samples of \taxi.\\
}
\end{minipage}
\hfill
\begin{minipage}{\columnwidth}
% \newcommand{\sv}{
% \fontsize{7pt}{7pt}\selectfont{\cellcolor[HTML]{4D908E}{\textsf{SV}\xspace}}}
% \newcommand{\pc}{\fontsize{7pt}{7pt}\selectfont{\cellcolor[HTML]{FEDC97}{\textsf{LP}\xspace}}}
% \newcommand{\ws}{\fontsize{7pt}{7pt}\selectfont{\cellcolor[HTML]{90BE6D}{\textsf{WS}\xspace}}}

% % Please add the following required packages to your document preamble:
% % \usepackage{graphicx}
% % Please add the following required packages to your document preamble:
% % \usepackage{graphicx}
\vspace{+0.5cm}
\resizebox{\columnwidth}{!}{%
\huge
\begin{tabular}{r|ccccccc|@{\hspace{5pt}}|ccccccc|}
\cline{2-15}
 &
  \multicolumn{7}{c|@{\hspace{5pt}}|}{Patrol} &
  \multicolumn{7}{c|}{Taxi} \\\hhline{-==============}
\multicolumn{1}{|r|}{\textbf{\% Sample}} &
  \multicolumn{1}{c|}{\textbf{1\%}} &
  \multicolumn{1}{c|}{\textbf{5\%}} &
  \multicolumn{1}{c|}{\textbf{15\%}} &
  \multicolumn{1}{c|}{\textbf{25\%}} &
  \multicolumn{1}{c|}{\textbf{50\%}} &
  \multicolumn{1}{c|}{\textbf{75\%}} &
  \textbf{100\%} &
  \multicolumn{1}{c|}{\textbf{1\%}} &
  \multicolumn{1}{c|}{\textbf{5\%}} &
  \multicolumn{1}{c|}{\textbf{15\%}} &
  \multicolumn{1}{c|}{\textbf{25\%}} &
  \multicolumn{1}{c|}{\textbf{50\%}} &
  \multicolumn{1}{c|}{\textbf{75\%}} &
  \textbf{100\%}\\ \cline{1-15}
  \multicolumn{1}{|r|}{\textbf{\# Rows (M)}} &
  \multicolumn{1}{c|}{\textbf{0.2}} &
  \multicolumn{1}{c|}{\textbf{1.2}} &
  \multicolumn{1}{c|}{\textbf{4.5}} &
  \multicolumn{1}{c|}{\textbf{6.7}} &
  \multicolumn{1}{c|}{\textbf{13.5}} &
  \multicolumn{1}{c|}{\textbf{20.2}} &
  \textbf{27} &
  \multicolumn{1}{c|}{\textbf{0.7}} &
  \multicolumn{1}{c|}{\textbf{3.8}} &
  \multicolumn{1}{c|}{\textbf{11.5}} &
  \multicolumn{1}{c|}{\textbf{19.2}} &
  \multicolumn{1}{c|}{\textbf{38.8}} &
  \multicolumn{1}{c|}{\textbf{57.7}} &
  \textbf{77}\\ \hline \hline
\multicolumn{1}{|r|}{Pandas} &
  \multicolumn{1}{c|}{\pc} &
  \multicolumn{1}{c|}{\pc} &
  \multicolumn{1}{c|}{\pc} &
  \multicolumn{1}{c|}{\pc} &
  \multicolumn{1}{c|}{\ws} &
  \multicolumn{1}{c|}{\ws} &
  \ws &
  \multicolumn{1}{c|}{\pc} &
  \multicolumn{1}{c|}{\pc} &
  \multicolumn{1}{c|}{\ws} &
  \multicolumn{1}{c|}{\ws} &
  \multicolumn{1}{c|}{\sv} &
  \multicolumn{1}{c|}{\sv} &
  \xmark\\ \hline
\multicolumn{1}{|r|}{SparkPD} &
  \multicolumn{1}{c|}{\ws} &
  \multicolumn{1}{c|}{\ws} &
  \multicolumn{1}{c|}{\ws} &
  \multicolumn{1}{c|}{\ws} &
  \multicolumn{1}{c|}{\ws} &
  \multicolumn{1}{c|}{\ws} &
  \ws &
  \multicolumn{1}{c|}{\ws} &
  \multicolumn{1}{c|}{\ws} &
  \multicolumn{1}{c|}{\ws} &
  \multicolumn{1}{c|}{\ws} &
  \multicolumn{1}{c|}{\ws} &
  \multicolumn{1}{c|}{\ws} &
  \ws\\ \hline
\multicolumn{1}{|r|}{SparkSQL} &
  \multicolumn{1}{c|}{\pc} &
  \multicolumn{1}{c|}{\pc} &
  \multicolumn{1}{c|}{\pc} &
  \multicolumn{1}{c|}{\pc} &
  \multicolumn{1}{c|}{\pc} &
  \multicolumn{1}{c|}{\pc} &
  \pc &
  \multicolumn{1}{c|}{\pc} &
  \multicolumn{1}{c|}{\pc} &
  \multicolumn{1}{c|}{\pc} &
  \multicolumn{1}{c|}{\pc} &
  \multicolumn{1}{c|}{\pc} &
  \multicolumn{1}{c|}{\pc} &
  \pc\\ \hline
\multicolumn{1}{|r|}{ModinD} &
  \multicolumn{1}{c|}{\pc} &
  \multicolumn{1}{c|}{\pc} &
  \multicolumn{1}{c|}{\pc} &
  \multicolumn{1}{c|}{\ws} &
  \multicolumn{1}{c|}{\sv} &
  \multicolumn{1}{c|}{\sv} &
  \sv &
  \multicolumn{1}{c|}{\pc} &
  \multicolumn{1}{c|}{\pc} &
  \multicolumn{1}{c|}{\pc} &
  \multicolumn{1}{c|}{\ws}  & \multicolumn{1}{c|}{\sv} &
  \multicolumn{1}{c|}{\xmark} &
  \xmark\\ \hline
\multicolumn{1}{|r|}{ModinR} &
  \multicolumn{1}{c|}{\pc} &
  \multicolumn{1}{c|}{\pc} &
  \multicolumn{1}{c|}{\pc} &
  \multicolumn{1}{c|}{\pc} &
  \multicolumn{1}{c|}{\ws} &
  \multicolumn{1}{c|}{\ws} &
  \ws &
  \multicolumn{1}{c|}{\pc} &
  \multicolumn{1}{c|}{\pc} &
  \multicolumn{1}{c|}{\pc} &
  \multicolumn{1}{c|}{\pc} &
  \multicolumn{1}{c|}{\ws} &
  \multicolumn{1}{c|}{\ws} &
  \ws\\ \hline
\multicolumn{1}{|r|}{Polars} &
  \multicolumn{1}{c|}{\pc} &
  \multicolumn{1}{c|}{\pc} &
  \multicolumn{1}{c|}{\pc} &
  \multicolumn{1}{c|}{\ws} &
  \multicolumn{1}{c|}{\ws} &
  \multicolumn{1}{c|}{\ws} &
  \ws &
  \multicolumn{1}{c|}{\pc} &
  \multicolumn{1}{c|}{\pc} &
  \multicolumn{1}{c|}{\ws} &
  \multicolumn{1}{c|}{\ws} &
  \multicolumn{1}{c|}{\ws} &
  \multicolumn{1}{c|}{\sv} &
  \sv\\ \hline
% \multicolumn{1}{|r|}{cuDF} &
%   \multicolumn{1}{c|}{\pc} &
%   \multicolumn{1}{c|}{\pc} &
%   \multicolumn{1}{c|}{\pc} &
%   \multicolumn{1}{c|}{\pc} &
%   \multicolumn{1}{c|}{\pc} &
%   \multicolumn{1}{c|}{\pc} &
%   \pc &
%   \multicolumn{1}{c|}{\pc} &
%   \multicolumn{1}{c|}{\pc} &
%   \multicolumn{1}{c|}{\pc} &
%   \multicolumn{1}{c|}{\ws} &
%   \multicolumn{1}{c|}{\ws} &
%   \multicolumn{1}{c|}{\ws} &
%   \ws\\ \hline
\multicolumn{1}{|r|}{Vaex} &
  \multicolumn{1}{c|}{\pc} &
  \multicolumn{1}{c|}{\pc} &
  \multicolumn{1}{c|}{\pc} &
  \multicolumn{1}{c|}{\ws} &
  \multicolumn{1}{c|}{\ws} &
  \multicolumn{1}{c|}{\ws} &
  \ws &
  \multicolumn{1}{c|}{\pc} &
  \multicolumn{1}{c|}{\pc} &
  \multicolumn{1}{c|}{\pc} &
  \multicolumn{1}{c|}{\ws} &
  \multicolumn{1}{c|}{\ws} &
  \multicolumn{1}{c|}{\ws} &
  \ws\\ \hline
\multicolumn{1}{|r|}{DataTable} &
  \multicolumn{1}{c|}{\pc} &
  \multicolumn{1}{c|}{\pc} &
  \multicolumn{1}{c|}{\pc} &
  \multicolumn{1}{c|}{\pc} &
  \multicolumn{1}{c|}{\pc} &
  \multicolumn{1}{c|}{\ws} & 
  \ws &
  \multicolumn{1}{c|}{\pc} &
  \multicolumn{1}{c|}{\pc} &
  \multicolumn{1}{c|}{\pc} &
  \multicolumn{1}{c|}{\pc} &
  \multicolumn{1}{c|}{\ws} &
  \multicolumn{1}{c|}{\ws} &
  \ws\\ \hline
  \multicolumn{15}{c}{\rule{0pt}{3ex}\colorbox[HTML]{90BE6D}{\color[HTML]{90BE6D}III} Laptop \hspace{0.25cm} \colorbox[HTML]{FEDC97}{\color[HTML]{FEDC97}III} Workstation \hspace{0.25cm} \colorbox[HTML]{F9844A}{\color[HTML]{F9844A}III} Server}
\end{tabular}
}
%}
\vspace{+0.5cm}
\caption{Minimum machine configuration for running the entire pipeline on incremental dataset samples.
%\colorbox[HTML]{90BE6D}{Laptop}, \colorbox[HTML]{FEDC97}{Workstation}, \colorbox[HTML]{f9844a}{Server}. See Table \ref{tab:machineconfiguration} for the detailed configurations.
}
\label{tab:scalability}
\end{minipage}
\end{table*}


==> input/images/load_tpch.tex <==
\begin{figure}[ht]
\centering
\includegraphics[width=0.5\columnwidth]{input/images/tpch_load.pdf}

\caption{TPC-H 10GB - Average Load Time}
\label{fig:load_time}
\end{figure}

==> input/images/memory/memory.tex <==
\begin{figure}[ht]
    \begin{subfigure}[b]{0.20\textwidth}
         \centering
         \includegraphics[width=\linewidth]{input/images/memory/athlete.pdf}
         \vspace*{-0.6cm}
         \caption{Athlete}
         \label{fig:memory_athlete}
    \end{subfigure}
    \hfill
        \begin{subfigure}[b]{0.20\textwidth}
         \centering
         \includegraphics[width=\linewidth]{input/images/memory/loan.pdf}
         \vspace*{-0.6cm}
         \caption{Loan}
         \label{fig:memory_loan}
    \end{subfigure}
    \hfill
        \begin{subfigure}[b]{0.20\textwidth}
         \centering
         \includegraphics[width=\linewidth]{input/images/memory/state_patrol.pdf}
                 \vspace*{-0.61cm}
        \caption{Patrol}
         \label{fig:memory_patrol}
    \end{subfigure}
    \hfill
        \begin{subfigure}[b]{0.20\textwidth}
         \centering
         \includegraphics[width=\linewidth]{input/images/memory/nyc_taxi.pdf}
        \vspace*{-0.6cm}
         \caption{Taxi}
         \label{fig:memory_taxi}
    \end{subfigure}
\caption{Peak Memory Consumption (GB)}
\label{fig:memory_peak}
\end{figure}

==> input/images/tab4/apply_comparison.tex <==
\begin{figure}[ht]
\centering
\begin{subfigure}{0.45\linewidth}
         \includegraphics[width=0.95\linewidth]{input/images/tab4/state_patrol_apply.pdf}
\end{subfigure}
\begin{subfigure}{0.45\linewidth}
         \includegraphics[width=0.95\linewidth]{input/images/tab4/nyc_taxi_apply.pdf}
\end{subfigure}
\caption{Average runtime for the \emph{apply} preparator on \patrol and \taxi (only libraries not raising OoM issues).}
\label{fig:apply_core}
\end{figure}

==> input/images/tab5/tab5.tex <==
\begin{figure}
\begin{subfigure}{\columnwidth}
         \centering
         \includegraphics[width=0.8\textwidth]{input/images/tab5/legend.pdf}
\end{subfigure}
\begin{subfigure}{0.45\columnwidth}
    \includegraphics[width=0.85\textwidth]{input/images/tab5/Athlete.pdf}
    \caption{Image A}
\end{subfigure}
\begin{subfigure}{0.45\columnwidth}
    \includegraphics[width=0.85\textwidth]{input/images/tab5/Loan.pdf}
    \caption{Image A}
\end{subfigure}
\begin{subfigure}{0.45\columnwidth}
    \includegraphics[width=0.85\textwidth]{input/images/tab5/Patrol.pdf}
    \caption{Image A}
\end{subfigure}
\begin{subfigure}{0.45\columnwidth}
    \includegraphics[width=0.85\textwidth]{input/images/tab5/Taxi.pdf}
    \caption{Image A}
\end{subfigure}
\end{figure}

==> input/tables/dataset_characteristics.tex <==
\begin{table}[ht]
\caption{Features of the selected datasets.}
\label{tab:dataset}
\begin{adjustbox}{max width=\columnwidth}
\begin{tabular}{r|cccc|}
\cline{2-5}
                                            & \textbf{Athlete} & \textbf{Loan} & \textbf{Patrol} & \textbf{Taxi} \\ \hhline{-====}
\multicolumn{1}{|r|}{CSV Size (GB)}         & 0.03             & 1.6           & 6.7             & 10.9          \\ \hline
\multicolumn{1}{|r|}{\# Rows ($\times10^{6}$)} & 0.2              & 2             & 27              & 77            \\ \hline
\multicolumn{1}{|r|}{\# Columns}               & 15               & 151           & 34              & 18            \\ \hline
\multicolumn{1}{|r|}{\# Num - Str - Bool}     & 5-10-0                & 113-38-0           & 5-27-2   & 15-3-0            \\ \hline
% \multicolumn{1}{|r|}{\# Objects}               & 10               & 38            & 27              & 3             \\ \hline
% \multicolumn{1}{|r|}{\# Boolean}               & 0                & 0             & 2               & 0             \\ \hline
\multicolumn{1}{|r|}{\% Null}                  &         9\%         & 31\%           &    22\%             &  0\%             \\ \hline
\multicolumn{1}{|r|}{Str Len Range}           & (1, 108)         & (1, 3988)     & (1, 2293)       & (1, 19)       \\ \hline
\end{tabular}
\end{adjustbox}  
\end{table}

==> input/tables/machine_config.tex <==
\begin{table}[ht]
\caption{Specifications of each machine configuration.}
\label{tab:machineconfiguration}
\begin{adjustbox}{max width=\columnwidth}
\begin{tabular}{r|ccc|}
\cline{2-4}
                                & \textbf{Laptop} & \textbf{Workstation} & \textbf{Server} \\ \hhline{-===}
\multicolumn{1}{|r|}{\# CPUs}   & 8               & 16                   & 24              \\ \hline
\multicolumn{1}{|r|}{\# RAM (GB)} & 16              & 64                   & 128             \\ \hline
\multicolumn{1}{|r|}{Dask (workers - threads)} & 4-8              & 4-16                   & 6-24             \\ \hline
\multicolumn{1}{|r|}{Ray (workers)} & 8              & 16                   & 24             \\ \hline
\end{tabular}
\end{adjustbox}
\end{table}

==> input/tables/scalability_table.tex <==
\newcommand{\sv}{\selectfont{\cellcolor[HTML]{4D908E}{\textsf{SV}\xspace}}}
\newcommand{\pc}{\selectfont{\cellcolor[HTML]{FEDC97}{\textsf{LP}\xspace}}}
\newcommand{\ws}{\selectfont{\cellcolor[HTML]{90BE6D}{\textsf{WS}\xspace}}}
% \newcommand{\sv}{
% \fontsize{7pt}{7pt}\selectfont{\cellcolor[HTML]{4D908E}{\textsf{SV}\xspace}}}
% \newcommand{\pc}{\fontsize{7pt}{7pt}\selectfont{\cellcolor[HTML]{FEDC97}{\textsf{LP}\xspace}}}
% \newcommand{\ws}{\fontsize{7pt}{7pt}\selectfont{\cellcolor[HTML]{90BE6D}{\textsf{WS}\xspace}}}

% % Please add the following required packages to your document preamble:
% % \usepackage{graphicx}
% % Please add the following required packages to your document preamble:
% % \usepackage{graphicx}
\begin{table}[ht]
\caption{{\color{red}
Rev4(D16) The color coding in Table 3 could help the interpretation if Laptop, Workstation, and Server were colored green, yellow, and orange (or similar) to indicate "can handle easily," "with moderate effort," and "only with major effort," respectively.
} Minimum machine configuration for running the entire pipeline on incremental dataset samples. \colorbox[HTML]{FEDC97}{Laptop}, \colorbox[HTML]{90BE6D}{Workstation}, \colorbox[HTML]{4D908E}{Server}. See Table \ref{tab:machineconfiguration} for the detailed configurations.}
\label{tab:scalability}
% \resizebox{\textwidth}{!}{%
\resizebox{\columnwidth}{!}{%
\begin{tabular}{r|ccccccc||ccccccc|}
\cline{2-15}
 &
  \multicolumn{7}{c||}{Patrol} &
  \multicolumn{7}{c|}{Taxi} \\ \hhline{-==============}
\multicolumn{1}{|r|}{\textbf{\% Sample}} &
  \multicolumn{1}{c|}{\textbf{1\%}} &
  \multicolumn{1}{c|}{\textbf{5\%}} &
  \multicolumn{1}{c|}{\textbf{15\%}} &
  \multicolumn{1}{c|}{\textbf{25\%}} &
  \multicolumn{1}{c|}{\textbf{50\%}} &
  \multicolumn{1}{c|}{\textbf{75\%}} &
  \textbf{100\%} &
  \multicolumn{1}{c|}{\textbf{1\%}} &
  \multicolumn{1}{c|}{\textbf{5\%}} &
  \multicolumn{1}{c|}{\textbf{15\%}} &
  \multicolumn{1}{c|}{\textbf{25\%}} &
  \multicolumn{1}{c|}{\textbf{50\%}} &
  \multicolumn{1}{c|}{\textbf{75\%}} &
  \textbf{100\%}\\ \cline{1-15}
  \multicolumn{1}{|r|}{\textbf{\# Rows (M)}} &
  \multicolumn{1}{c|}{\textbf{0.2}} &
  \multicolumn{1}{c|}{\textbf{1.2}} &
  \multicolumn{1}{c|}{\textbf{4.5}} &
  \multicolumn{1}{c|}{\textbf{6.7}} &
  \multicolumn{1}{c|}{\textbf{13.5}} &
  \multicolumn{1}{c|}{\textbf{20.2}} &
  \textbf{27} &
  \multicolumn{1}{c|}{\textbf{0.7}} &
  \multicolumn{1}{c|}{\textbf{3.8}} &
  \multicolumn{1}{c|}{\textbf{11.5}} &
  \multicolumn{1}{c|}{\textbf{19.2}} &
  \multicolumn{1}{c|}{\textbf{38.8}} &
  \multicolumn{1}{c|}{\textbf{57.7}} &
  \textbf{77}\\ \hline \hline
\multicolumn{1}{|r|}{Pandas} &
  \multicolumn{1}{c|}{\pc} &
  \multicolumn{1}{c|}{\pc} &
  \multicolumn{1}{c|}{\pc} &
  \multicolumn{1}{c|}{\pc} &
  \multicolumn{1}{c|}{\ws} &
  \multicolumn{1}{c|}{\ws} &
  \ws &
  \multicolumn{1}{c|}{\pc} &
  \multicolumn{1}{c|}{\pc} &
  \multicolumn{1}{c|}{\ws} &
  \multicolumn{1}{c|}{\ws} &
  \multicolumn{1}{c|}{\sv} &
  \multicolumn{1}{c|}{\sv} &
  \xmark\\ \hline
\multicolumn{1}{|r|}{SparkPD} &
  \multicolumn{1}{c|}{\ws} &
  \multicolumn{1}{c|}{\ws} &
  \multicolumn{1}{c|}{\ws} &
  \multicolumn{1}{c|}{\ws} &
  \multicolumn{1}{c|}{\ws} &
  \multicolumn{1}{c|}{\ws} &
  \ws &
  \multicolumn{1}{c|}{\ws} &
  \multicolumn{1}{c|}{\ws} &
  \multicolumn{1}{c|}{\ws} &
  \multicolumn{1}{c|}{\ws} &
  \multicolumn{1}{c|}{\ws} &
  \multicolumn{1}{c|}{\ws} &
  \ws\\ \hline
\multicolumn{1}{|r|}{SparkSQL} &
  \multicolumn{1}{c|}{\pc} &
  \multicolumn{1}{c|}{\pc} &
  \multicolumn{1}{c|}{\pc} &
  \multicolumn{1}{c|}{\pc} &
  \multicolumn{1}{c|}{\pc} &
  \multicolumn{1}{c|}{\pc} &
  \pc &
  \multicolumn{1}{c|}{\pc} &
  \multicolumn{1}{c|}{\pc} &
  \multicolumn{1}{c|}{\pc} &
  \multicolumn{1}{c|}{\pc} &
  \multicolumn{1}{c|}{\pc} &
  \multicolumn{1}{c|}{\pc} &
  \pc\\ \hline
\multicolumn{1}{|r|}{ModinD} &
  \multicolumn{1}{c|}{\pc} &
  \multicolumn{1}{c|}{\pc} &
  \multicolumn{1}{c|}{\pc} &
  \multicolumn{1}{c|}{\ws} &
  \multicolumn{1}{c|}{\sv} &
  \multicolumn{1}{c|}{\sv} &
  \sv &
  \multicolumn{1}{c|}{\pc} &
  \multicolumn{1}{c|}{\pc} &
  \multicolumn{1}{c|}{\pc} &
  \multicolumn{1}{c|}{\ws}  & \multicolumn{1}{c|}{\sv} &
  \multicolumn{1}{c|}{\xmark} &
  \xmark\\ \hline
\multicolumn{1}{|r|}{ModinR} &
  \multicolumn{1}{c|}{\pc} &
  \multicolumn{1}{c|}{\pc} &
  \multicolumn{1}{c|}{\pc} &
  \multicolumn{1}{c|}{\pc} &
  \multicolumn{1}{c|}{\ws} &
  \multicolumn{1}{c|}{\ws} &
  \ws &
  \multicolumn{1}{c|}{\pc} &
  \multicolumn{1}{c|}{\pc} &
  \multicolumn{1}{c|}{\pc} &
  \multicolumn{1}{c|}{\pc} &
  \multicolumn{1}{c|}{\ws} &
  \multicolumn{1}{c|}{\ws} &
  \ws\\ \hline
\multicolumn{1}{|r|}{Polars} &
  \multicolumn{1}{c|}{\pc} &
  \multicolumn{1}{c|}{\pc} &
  \multicolumn{1}{c|}{\pc} &
  \multicolumn{1}{c|}{\ws} &
  \multicolumn{1}{c|}{\ws} &
  \multicolumn{1}{c|}{\ws} &
  \ws &
  \multicolumn{1}{c|}{\pc} &
  \multicolumn{1}{c|}{\pc} &
  \multicolumn{1}{c|}{\ws} &
  \multicolumn{1}{c|}{\ws} &
  \multicolumn{1}{c|}{\ws} &
  \multicolumn{1}{c|}{\sv} &
  \sv\\ \hline
% \multicolumn{1}{|r|}{cuDF} &
%   \multicolumn{1}{c|}{\pc} &
%   \multicolumn{1}{c|}{\pc} &
%   \multicolumn{1}{c|}{\pc} &
%   \multicolumn{1}{c|}{\pc} &
%   \multicolumn{1}{c|}{\pc} &
%   \multicolumn{1}{c|}{\pc} &
%   \pc &
%   \multicolumn{1}{c|}{\pc} &
%   \multicolumn{1}{c|}{\pc} &
%   \multicolumn{1}{c|}{\pc} &
%   \multicolumn{1}{c|}{\ws} &
%   \multicolumn{1}{c|}{\ws} &
%   \multicolumn{1}{c|}{\ws} &
%   \ws\\ \hline
\multicolumn{1}{|r|}{Vaex} &
  \multicolumn{1}{c|}{\pc} &
  \multicolumn{1}{c|}{\pc} &
  \multicolumn{1}{c|}{\pc} &
  \multicolumn{1}{c|}{\ws} &
  \multicolumn{1}{c|}{\ws} &
  \multicolumn{1}{c|}{\ws} &
  \ws &
  \multicolumn{1}{c|}{\pc} &
  \multicolumn{1}{c|}{\pc} &
  \multicolumn{1}{c|}{\pc} &
  \multicolumn{1}{c|}{\ws} &
  \multicolumn{1}{c|}{\ws} &
  \multicolumn{1}{c|}{\ws} &
  \ws\\ \hline
\multicolumn{1}{|r|}{Datatable} &
  \multicolumn{1}{c|}{\pc} &
  \multicolumn{1}{c|}{\pc} &
  \multicolumn{1}{c|}{\pc} &
  \multicolumn{1}{c|}{\pc} &
  \multicolumn{1}{c|}{\pc} &
  \multicolumn{1}{c|}{\ws} & 
  \ws &
  \multicolumn{1}{c|}{\pc} &
  \multicolumn{1}{c|}{\pc} &
  \multicolumn{1}{c|}{\pc} &
  \multicolumn{1}{c|}{\pc} &
  \multicolumn{1}{c|}{\ws} &
  \multicolumn{1}{c|}{\ws} &
  \ws\\ \hline
\end{tabular}
}
%}
\end{table}


==> input/tables/test_table.tex <==
% \usepackage{tabularray}
\renewcommand{\arraystretch}{2}
\begin{table}
\centering
\fontsize{100}{102}\selectfont
\begin{adjustbox}{max width=\columnwidth}
\begin{tabular}{|r|r|r|c|c|c|c|c|c|c|c|}
% \usepackage{array}
method               & cuDF  & dt     & mdDD   & mdR   & pd     & pd2   & pl     & psPD   & psSQL  & vx       \\
calc\_column         & 2.64  & 8.706  & 9.329  & 1.527 & 4.7    & 4.483 & 6.524  & 16.019 & 0.495  & 0.002    \\
cast\_columns\_types & 0.002 & 0.001  & 1.852  & 0.3   & 0.539  & 0.493 & 8.789  & 10.78  & 0.296  & 0.352    \\
delete\_columns      & 0.011 & 0.001  & 0.011  & 0.009 & 0.04   & 0.039 & 0.029  & 4.255  & 0.712  & 0.006    \\
drop\_duplicates     & 0.058 & 11.295 & 8.834  & 2.497 & 0.42   & 0.408 & 10.172 & 17.79  & 1.946  & 53.633   \\
fill\_nan            & 0.002 & 0.019  & 1.741  & 0.276 & 0.055  & 0.019 & 10.109 & 16.701 & 0.982  & 0.009    \\
get\_columns         & 0.001 & 0.001  & 0.001  & 0.001 & 0.001  & 0.001 & 0.001  & 0.577  & 0.582  & 0.001    \\
groupby              & 0.011 & 0.319  & 8.225  & 6.831 & 0.386  & 0.366 & 10.091 & 16.533 & 1.063  & 40.806   \\
join                 & 0.024 & 0.044  & 1.483  & 0.292 & 0.147  & 0.078 & 13.215 & 9.608  & 2.617  & 3.342    \\
load\_dataset        & 1.033 & 0.09   & 2.066  & 3.958 & 0.898  & 0.857 & 1.28   & 9.47   & 4.857  & 0.139    \\
locate\_null\_values & 0.016 & 0.002  & 1.767  & 4.54  & 0.861  & 0.275 & 0.001  & 1.422  & 0.431  & 0.965    \\
pivot                & 0.91  & 0.517  & 5.629  & 0.895 & 0.187  & 0.114 & 20.023 & 19.864 & 3.557  & 24.655   \\

\end{tabular}
\end{adjustbox}
\end{table}
